Revealing and Mitigating Transmittance and Reflectance Errors in Integrating-Sphere Characterization of High-Albedo Scattering Media

Accurate optical characterization of high-albedo scattering media is fundamentally limited by integrating-sphere measurement errors. Scattering events spatially redistribute photons, leading to lateral beam spread and angular divergence that bias measured reflectance and transmittance. Here, we investigate these deviations, which are quantified and interpreted by using the point spread function (PSF), guided by the radiative transfer equation. Experiments and Monte Carlo modelling show that the widely used external-mount integrating-sphere configuration introduces systematic, configuration-dependent errors that become pronounced when scattering-induced lateral spreading is substantial. Using a normalised PSF to quantify photon redistribution, we map the characteristic lateral spreading length across a broad $(\taus,g)$ parameter space in the high-albedo limit, providing a basis for evaluating errors in specific measurement geometries. We further quantify the influence of measurement geometry and show that, in the pencil-beam limit, maintaining $L/D_{\mathrm{port}}\lesssim 0.01$ reduces the discrepancy arising from the finite collection aperture to approximately \qty{1}{\percent}. In addition, we introduce an internal-mount integrating-sphere protocol that suppresses scattering-related losses and yields transmittance and reflectance measurements in good agreement with theoretical predictions. Overall, our work helps users of integrating-sphere measurements identify scattering-related errors and improve the reliability of transmittance and reflectance characterization across a wide range of application areas.

==> macros.tex <==
% macros.tex

\RequirePackage{xparse}
\providecommand{\threesubsection}[1]{\subsection{#1}}


% Custom symbols
\NewDocumentCommand{\mus}{o}{\ensuremath{\mu_\text{s}\IfValueT{#1}{^{#1}}}}
\NewDocumentCommand{\musp}{o}{\ensuremath{\mu_\text{s}^\prime\IfValueT{#1}{^{#1}}}}
\NewDocumentCommand{\mua}{o}{\ensuremath{\mu_\text{a}\IfValueT{#1}{^{#1}}}}
\NewDocumentCommand{\ellt}{o}{\ensuremath{\ell_\text{t}\IfValueT{#1}{^{#1}}}}
\NewDocumentCommand{\taus}{o}{\ensuremath{\tau_\text{s}\IfValueT{#1}{^{#1}}}}
\NewDocumentCommand{\tausp}{o}{\ensuremath{\tau_\text{s}^\prime\IfValueT{#1}{^{#1}}}}
\NewDocumentCommand{\taua}{o}{\ensuremath{\tau_\text{a}\IfValueT{#1}{^{#1}}}}


